On the Power of Heuristics in Temporal Graphs

Dynamic graph datasets often exhibit strong temporal patterns, such as recency, which prioritizes recent interactions, and popularity, which favors frequently occurring nodes. We demonstrate that simple heuristics leveraging only these patterns can perform on par or outperform state-of-the-art neural network models under standard evaluation protocols. To further explore these dynamics, we introduce metrics that quantify the impact of recency and popularity across datasets. Our experiments on BenchTemp and the Temporal Graph Benchmark show that our approaches achieve state-of-the-art performance across all datasets in the latter and secure top ranks on multiple datasets in the former. These results emphasize the importance of refined evaluation schemes to enable fair comparisons and promote the development of more robust temporal graph models. Additionally, they reveal that current deep learning methods often struggle to capture the key patterns underlying predictions in real-world temporal graphs. For reproducibility, we have made our code publicly available.

==> auc_table.tex <==
\begin{tabular}{lrrrr}
\toprule
\textbf{Dataset} & \multicolumn{2}{c}{\textbf{Global Recency}} & \multicolumn{2}{c}{\textbf{Local Recency}} \\
                 & $R^+$            & $R^-$            & $R^+$            & $R^-$            \\
\midrule
\textbf{CanParl}            & 0.860          & 0.596          & 0.952          & 0.438          \\
\textbf{CollegeMsg}         & 0.922          & 0.922          & 0.991          & 0.708          \\
\textbf{Contacts}           & 0.981          & 0.773          & 0.985          & 0.975          \\
\textbf{DGraphFin}          & 0.481          & 0.302          & 1.000          & 0.000          \\
\textbf{Flights}            & 0.946          & 0.635          & 0.996          & 0.847          \\
\textbf{SocialEvo}          & 0.806          & 0.787          & 0.971          & 0.963          \\
\textbf{TaobaoLarge}        & 0.712          & 0.707          & 1.000          & 0.170          \\
\textbf{UNtrade}            & 0.996          & 0.630          & 0.975          & 0.924          \\
\textbf{UNvote}             & 0.987          & 0.706          & 0.983          & 0.958          \\
\textbf{USLegis}            & 0.848          & 0.681          & 0.859          & 0.572          \\
\textbf{YoutubeRedditLarge} & 0.942          & 0.940          & 1.000          & 0.330          \\
\textbf{enron}              & 0.839          & 0.834          & 0.961          & 0.873          \\
\textbf{lastfm}             & 0.690          & 0.690          & 0.934          & 0.861          \\
\textbf{mooc}               & 0.717          & 0.715          & 0.809          & 0.574          \\
\textbf{reddit}             & 0.880          & 0.880          & 0.994          & 0.927          \\
\textbf{taobao}             & 0.268          & 0.225          & 1.000          & 0.090          \\
\textbf{tgbl-coin}          & 0.935          & 0.935          & 0.997          & 0.869          \\
\textbf{tgbl-comment}       & 0.974          & 0.972          & 0.999          & 0.170          \\
\textbf{tgbl-flight}        & 0.976          & 0.679          & 0.996          & 0.968          \\
\textbf{tgbl-lastfm}        & 0.690          & 0.690          & 0.934          & 0.861          \\
\textbf{tgbl-review}        & 0.898          & 0.896          & 1.000          & 0.010          \\
\textbf{tgbl-subreddit}     & 0.880          & 0.880          & 0.994          & 0.927          \\
\textbf{tgbl-wiki}          & 0.909          & 0.909          & 0.994          & 0.889          \\
\textbf{uci}                & 0.922          & 0.922          & 0.991          & 0.708          \\
\textbf{wikipedia}          & 0.909          & 0.909          & 0.994          & 0.889          \\
\bottomrule
\end{tabular}

==> benchtemp_only_heuristics.tex <==
\begin{tabular}{lllllll}
\toprule
             & Heuristic &        Recency &                   NaN &                Popularity &       Recency &               Popularity \\
             & Locality &         Global &                   NaN &                    Global &         Local &                    Local \\
             & Model & global recency & all heuristics in one & global popularity tracker & local recency & local popularity tracker \\
Metric & Dataset &                &                       &                           &               &                          \\
\midrule
inductive & canparl &          0.629 &                 0.636 &                     0.627 &         0.653 &                    0.652 \\
             & collegemsg &          0.922 &                 0.934 &                     0.793 &         0.838 &                    0.835 \\
             & contact &          0.876 &                 0.977 &                     0.622 &         0.966 &                    0.939 \\
             & enron &          0.817 &                 0.936 &                     0.554 &          0.92 &                    0.909 \\
             & flights &          0.784 &                 0.927 &                     0.827 &         0.851 &                     0.85 \\
             & lastfm &          0.759 &                 0.909 &                     0.492 &         0.902 &                    0.889 \\
             & mooc &          0.694 &                 0.708 &                     0.531 &         0.665 &                    0.615 \\
             & reddit &          0.764 &                   1.0 &                     0.773 &         0.933 &                    0.933 \\
             & socialevo &          0.784 &                 0.951 &                     0.482 &         0.952 &                     0.86 \\
             & taobao &          0.215 &                 0.218 &                     0.197 &         0.521 &                    0.521 \\
             & uci &           0.92 &                 0.931 &                     0.781 &         0.835 &                    0.833 \\
             & untrade &          0.552 &                 0.635 &                     0.472 &         0.689 &                    0.595 \\
             & unvote &          0.518 &                 0.542 &                     0.375 &          0.64 &                    0.502 \\
             & uslegis &          0.604 &                  0.59 &                      0.37 &          0.57 &                    0.539 \\
             & wikipedia &          0.916 &                 0.963 &                     0.431 &         0.917 &                    0.917 \\
inductive new new & canparl &          0.554 &                 0.572 &                      0.56 &         0.641 &                    0.643 \\
             & collegemsg &          0.919 &                 0.933 &                     0.746 &         0.843 &                    0.841 \\
             & contact &          0.871 &                 0.977 &                     0.477 &         0.967 &                    0.955 \\
             & enron &          0.771 &                 0.961 &                     0.389 &         0.949 &                    0.953 \\
             & flights &          0.771 &                 0.916 &                     0.716 &         0.876 &                    0.876 \\
             & lastfm &          0.909 &                 0.965 &                     0.503 &         0.962 &                    0.962 \\
             & mooc &          0.673 &                 0.684 &                     0.318 &         0.652 &                    0.605 \\
             & reddit &            1.0 &                   1.0 &                     0.938 &         0.875 &                    0.875 \\
             & socialevo &           0.79 &                 0.946 &                     0.238 &         0.948 &                    0.906 \\
             & taobao &          0.167 &                 0.169 &                     0.128 &         0.522 &                    0.522 \\
             & uci &          0.915 &                 0.931 &                     0.727 &         0.839 &                    0.837 \\
             & untrade &          0.544 &                 0.604 &                     0.265 &         0.694 &                    0.722 \\
             & unvote &          0.512 &                 0.386 &                     0.147 &         0.633 &                    0.619 \\
             & uslegis &          0.495 &                 0.458 &                     0.162 &         0.539 &                    0.535 \\
             & wikipedia &          0.926 &                 0.977 &                      0.35 &         0.941 &                     0.94 \\
inductive new old & canparl &          0.648 &                 0.652 &                     0.641 &         0.657 &                    0.655 \\
             & collegemsg &          0.921 &                 0.932 &                     0.811 &         0.835 &                    0.832 \\
             & contact &          0.876 &                 0.977 &                      0.63 &         0.966 &                    0.938 \\
             & enron &          0.818 &                 0.932 &                     0.573 &         0.916 &                    0.902 \\
             & flights &          0.786 &                 0.928 &                     0.839 &         0.849 &                    0.847 \\
             & lastfm &          0.676 &                 0.876 &                     0.486 &         0.867 &                    0.845 \\
             & mooc &          0.696 &                 0.711 &                      0.56 &         0.667 &                    0.616 \\
             & reddit &          0.719 &                   1.0 &                     0.752 &         0.955 &                    0.955 \\
             & socialevo &          0.784 &                 0.951 &                     0.499 &         0.953 &                    0.856 \\
             & taobao &           0.27 &                 0.276 &                     0.277 &         0.521 &                    0.521 \\
             & uci &          0.921 &                 0.932 &                     0.799 &         0.833 &                    0.831 \\
             & untrade &          0.553 &                 0.633 &                     0.487 &         0.688 &                    0.584 \\
             & unvote &          0.518 &                 0.546 &                     0.388 &          0.64 &                    0.492 \\
             & uslegis &          0.639 &                 0.624 &                     0.446 &         0.581 &                     0.54 \\
             & wikipedia &          0.911 &                 0.957 &                     0.468 &         0.907 &                    0.906 \\
transductive & canparl &          0.723 &                 0.731 &                      0.72 &         0.727 &                    0.721 \\
             & collegemsg &          0.922 &                 0.951 &                     0.867 &         0.872 &                     0.87 \\
             & contact &          0.878 &                 0.982 &                     0.794 &         0.976 &                    0.956 \\
             & enron &          0.819 &                 0.927 &                     0.688 &         0.903 &                    0.896 \\
             & flights &          0.793 &                 0.965 &                     0.907 &         0.921 &                    0.922 \\
             & lastfm &          0.618 &                 0.898 &                     0.614 &         0.896 &                    0.872 \\
             & mooc &          0.742 &                 0.769 &                     0.677 &         0.728 &                     0.65 \\
             & reddit &          0.881 &                 0.976 &                     0.898 &         0.958 &                    0.958 \\
             & socialevo &          0.782 &                 0.957 &                     0.723 &         0.957 &                    0.908 \\
             & taobao &          0.635 &                 0.737 &                     0.754 &         0.663 &                    0.663 \\
             & uci &          0.927 &                 0.952 &                     0.881 &         0.875 &                    0.874 \\
             & untrade &          0.553 &                 0.731 &                     0.718 &         0.692 &                     0.72 \\
             & unvote &           0.52 &                 0.685 &                     0.642 &         0.648 &                    0.677 \\
             & uslegis &           0.77 &                 0.819 &                     0.713 &         0.772 &                    0.745 \\
             & wikipedia &          0.906 &                 0.982 &                     0.668 &         0.963 &                    0.963 \\
\bottomrule
\end{tabular}

==> benchtemp_results.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}crllllllllllll@{}}
\toprule
\multicolumn{1}{l}{}                & \multicolumn{1}{l}{} & \multicolumn{2}{c}{Recency}                            & \multicolumn{2}{c}{Popularity}                         & \multicolumn{1}{c}{Combined}         & \multicolumn{7}{c}{Baselines}                                                                                                                                                                \\
Metric                              & Dataset              & \multicolumn{1}{c}{Local} & \multicolumn{1}{c}{Global} & \multicolumn{1}{c}{Local} & \multicolumn{1}{c}{Global} & \multicolumn{1}{c}{LR-GR-LP-GP}      & \multicolumn{1}{c}{DyRep} & \multicolumn{1}{c}{Jodie} & \multicolumn{1}{c}{TGAT} & \multicolumn{1}{c}{TGN} & \multicolumn{1}{c}{NAT} & \multicolumn{1}{c}{CAWN} & \multicolumn{1}{c}{NeurTW} \\ \midrule
\multirow{15}{*}{inductive}         & canparl              & 0.6552 ± 0.0009           & 0.6269 ± 0.0015            & 0.6533 ± 0.0009           & 0.6298 ± 0.0027            & \multicolumn{1}{l|}{0.6317 ± 0.0019} & 0.5532 ± 0.0088           & 0.5012 ± 0.0155           & 0.5802 ± 0.0069          & 0.5727 ± 0.0268         & 0.6214 ± 0.0734         & 0.7154 ± 0.0967          & 0.8871 ± 0.0139            \\
                                    & collegemsg           & 0.838 ± 0.0007            & 0.9211 ± 0.0006            & 0.8356 ± 0.0005           & 0.7878 ± 0.0015            & \multicolumn{1}{l|}{0.9338 ± 0.0004} & 0.4838 ± 0.0116           & 0.5097 ± 0.0306           & 0.715 ± 0.0007           & 0.7770 ± 0.0522         & 0.9603 ± 0.0173         & 0.9163 ± 0.0038          & 0.9726 ± 0.0002            \\
                                    & contact              & 0.9658 ± 0.0003           & 0.8754 ± 0.0004            & 0.9385 ± 0.0002           & 0.6227 ± 0.0012            & \multicolumn{1}{l|}{0.9776 ± 0.0002} & 0.8650 ± 0.0431           & 0.9358 ± 0.0025           & 0.5571 ± 0.0047          & 0.952 ± 0.0056          & 0.9466 ± 0.0127         & 0.9691 ± 0.0031          & 0.9842 ± 0.0               \\
                                    & enron                & 0.9179 ± 0.0007           & 0.8111 ± 0.003             & 0.9102 ± 0.0028           & 0.5396 ± 0.0035            & \multicolumn{1}{l|}{0.9395 ± 0.0019} & 0.7120 ± 0.0600           & 0.8038 ± 0.0223           & 0.5529 ± 0.015           & 0.8159 ± 0.0231         & 0.9520 ± 0.0057         & 0.9162 ± 0.0016          & 0.9051 ± 0.0027            \\
                                    & flights              & 0.8512 ± 0.0002           & 0.7844 ± 0.001             & 0.8502 ± 0.0              & 0.8271 ± 0.0005            & \multicolumn{1}{l|}{0.9266 ± 0.0002} & 0.8689 ± 0.0128           & 0.9218 ± 0.0094           & 0.8321 ± 0.0041          & 0.9519 ± 0.0043         & 0.9827 ± 0.003          & 0.9834 ± 0.0001          & 0.9158 ± 0.0               \\
                                    & lastfm               & 0.9022 ± 0.0002           & 0.7595 ± 0.0005            & 0.889 ± 0.0003            & 0.4912 ± 0.0003            & \multicolumn{1}{l|}{0.9097 ± 0.0002} & 0.7990 ± 0.0444           & 0.8011 ± 0.0344           & 0.5196 ± 0.0144          & 0.8284 ± 0.0142         & 0.9139 ± 0.0038         & 0.9082 ± 0.0015          & 0.8840 ± 0.0               \\
                                    & mooc                 & 0.664 ± 0.0004            & 0.6941 ± 0.0009            & 0.6161 ± 0.0003           & 0.5333 ± 0.0011            & \multicolumn{1}{l|}{0.7068 ± 0.0003} & 0.8269 ± 0.0182           & 0.7779 ± 0.0575           & 0.7370 ± 0.006           & 0.8869 ± 0.0249         & 0.7325 ± 0.0433         & 0.9481 ± 0.0006          & 0.8045 ± 0.0224            \\
                                    & reddit               & 0.9333 ± 0.0              & 0.9037 ± 0.0419            & 0.9333 ± 0.0              & 0.7985 ± 0.0451            & \multicolumn{1}{l|}{0.9941 ± 0.0084} & 0.9583 ± 0.0004           & 0.9514 ± 0.0045           & 0.9651 ± 0.0002          & 0.9760 ± 0.0002         & 0.9906 ± 0.0034         & 0.9869 ± 0.0000          & 0.9802 ± 0.0011            \\
                                    & socialevo            & 0.9518 ± 0.0002           & 0.7856 ± 0.0002            & 0.8611 ± 0.0004           & 0.4814 ± 0.0016            & \multicolumn{1}{l|}{0.9519 ± 0.0009} & 0.9158 ± 0.0039           & 0.8963 ± 0.0228           & 0.6748 ± 0.0021          & 0.9244 ± 0.0084         & 0.896 ± 0.0164          & 0.9298 ± 0.0002          &                            \\
                                    & taobao               & 0.5213 ± 0.0              & 0.2128 ± 0.0008            & 0.5213 ± 0.0              & 0.2007 ± 0.0016            & \multicolumn{1}{l|}{0.219 ± 0.0008}  & 0.7026 ± 0.0006           & 0.701 ± 0.0013            & 0.5261 ± 0.0119          & 0.7017 ± 0.0026         & 0.9992 ± 0.0002         & 0.7737 ± 0.0027          & 0.8843 ± 0.0016            \\
                                    & uci                  & 0.8348 ± 0.0004           & 0.92 ± 0.0008              & 0.8328 ± 0.0002           & 0.7833 ± 0.0042            & \multicolumn{1}{l|}{0.9322 ± 0.0006} & 0.4297 ± 0.0428           & 0.7517 ± 0.0059           & 0.7024 ± 0.0048          & 0.8083 ± 0.0237         & 0.9622 ± 0.0167         & 0.9177 ± 0.0015          & 0.9686 ± 0.0031            \\
                                    & untrade              & 0.6907 ± 0.0011           & 0.5522 ± 0.0007            & 0.5942 ± 0.0012           & 0.4732 ± 0.0028            & \multicolumn{1}{l|}{}                & 0.6467 ± 0.0112           & 0.6727 ± 0.0132           &                          & 0.5977 ± 0.014          & 0.6475 ± 0.0664         & 0.7398 ± 0.0007          & 0.5915 ± 0.0328            \\
                                    & unvote               & 0.6385 ± 0.0013           & 0.5169 ± 0.0002            & 0.4986 ± 0.0008           & 0.3744 ± 0.0006            & \multicolumn{1}{l|}{}                & 0.4993 ± 0.0103           & 0.5121 ± 0.0005           & 0.4770 ± 0.0047          & 0.5881 ± 0.0118         & 0.779 ± 0.0082          & 0.5911 ± 0.0006          & 0.5860 ± 0.0               \\
                                    & uslegis              & 0.5764 ± 0.0038           & 0.6039 ± 0.0015            & 0.5387 ± 0.004            & 0.3754 ± 0.0028            & \multicolumn{1}{l|}{}                & 0.5980 ± 0.0097           & 0.5840 ± 0.0129           & 0.5568 ± 0.0078          & 0.6128 ± 0.0046         & 0.7453 ± 0.0286         & 0.9665 ± 0.0032          & 0.9708 ± 0.0009            \\
                                    & wikipedia            & 0.9173 ± 0.0001           & 0.9161 ± 0.0003            & 0.9169 ± 0.0001           & 0.4313 ± 0.0013            & \multicolumn{1}{l|}{0.963 ± 0.0005}  & 0.9099 ± 0.0031           & 0.9305 ± 0.0020           & 0.9343 ± 0.0031          & 0.9781 ± 0.0005         & 0.9962 ± 0.0026         & 0.9890 ± 0.0003          & 0.9904 ± 0.0002            \\
\multirow{15}{*}{inductive new new} & canparl              & 0.6426 ± 0.0036           & 0.5644 ± 0.0034            & 0.6441 ± 0.0              & 0.5611 ± 0.0001            & \multicolumn{1}{l|}{0.5657 ± 0.004}  & 0.4430 ± 0.0068           & 0.4347 ± 0.0090           & 0.5955 ± 0.0074          & 0.5625 ± 0.0396         & 0.5685 ± 0.0326         & 0.7005 ± 0.1241          & 0.8882 ± 0.0045            \\
                                    & collegemsg           & 0.843 ± 0.0013            & 0.9204 ± 0.0032            & 0.842 ± 0.0003            & 0.7293 ± 0.0027            & \multicolumn{1}{l|}{0.9312 ± 0.0014} & 0.5269 ± 0.0049           & 0.5320 ± 0.0269           & 0.7832 ± 0.0026          & 0.7969 ± 0.0111         & 0.9404 ± 0.0371         & 0.9304 ± 0.0024          & 0.9762 ± 0.0008            \\
                                    & contact              & 0.9682 ± 0.0006           & 0.8717 ± 0.0025            & 0.9521 ± 0.0018           & 0.4598 ± 0.0043            & \multicolumn{1}{l|}{0.9788 ± 0.0008} & 0.6602 ± 0.0395           & 0.7531 ± 0.0059           & 0.5449 ± 0.0056          & 0.9118 ± 0.0053         & 0.9495 ± 0.0034         & 0.9652 ± 0.0012          & 0.9820 ± 0.0               \\
                                    & enron                & 0.952 ± 0.0044            & 0.7725 ± 0.0043            & 0.9528 ± 0.0006           & 0.4036 ± 0.0086            & \multicolumn{1}{l|}{0.9657 ± 0.0014} & 0.6571 ± 0.0521           & 0.6800 ± 0.0017           & 0.5310 ± 0.0179          & 0.7644 ± 0.0179         & 0.9687 ± 0.0051         & 0.9609 ± 0.0051          & 0.9387 ± 0.0000            \\
                                    & flights              & 0.8759 ± 0.0001           & 0.7709 ± 0.0025            & 0.8765 ± 0.0              & 0.7171 ± 0.0032            & \multicolumn{1}{l|}{0.9176 ± 0.0006} & 0.8900 ± 0.0266           & 0.9303 ± 0.0083           & 0.8570 ± 0.0056          & 0.9652 ± 0.0022         & 0.9905 ± 0.0014         & 0.9873 ± 0.0009          & 0.9411 ± 0.0               \\
                                    & lastfm               & 0.962 ± 0.0001            & 0.9103 ± 0.0003            & 0.9619 ± 0.0006           & 0.5002 ± 0.0014            & \multicolumn{1}{l|}{0.9661 ± 0.0003} & 0.8683 ± 0.0160           & 0.8852 ± 0.0090           & 0.5092 ± 0.0333          & 0.8754 ± 0.0011         & 0.9743 ± 0.0015         & 0.9697 ± 0.0002          & 0.9628 ± 0.0               \\
                                    & mooc                 & 0.6468 ± 0.0027           & 0.6689 ± 0.0034            & 0.6127 ± 0.0003           & 0.3137 ± 0.0089            & \multicolumn{1}{l|}{0.6884 ± 0.0011} & 0.7217 ± 0.0178           & 0.7065 ± 0.0165           & 0.7403 ± 0.0057          & 0.8762 ± 0.0038         & 0.6562 ± 0.0287         & 0.9422 ± 0.0003          & 0.8048 ± 0.0087            \\
                                    & reddit               & 0.875 ± 0.0               & 0.9375 ± 0.0884            & 0.875 ± 0.0               & 0.9792 ± 0.0295            & \multicolumn{1}{l|}{1.0 ± 0.0}       & 0.9525 ± 0.0050           & 0.9381 ± 0.0090           & 0.9597 ± 0.0043          & 0.9811 ± 0.0004         & 0.9954 ± 0.0011         & 0.9952 ± 0.0016          & 0.9875 ± 0.0004            \\
                                    & socialevo            & 0.9507 ± 0.0014           & 0.7843 ± 0.0061            & 0.9009 ± 0.0013           & 0.2373 ± 0.004             & \multicolumn{1}{l|}{0.9497 ± 0.0014} & 0.7740 ± 0.0215           & 0.6484 ± 0.0491           & 0.4659 ± 0.0068          & 0.8791 ± 0.0045         & 0.9275 ± 0.0471         & 0.9318 ± 0.0003          &                            \\
                                    & taobao               & 0.5215 ± 0.0              & 0.1639 ± 0.0011            & 0.5215 ± 0.0              & 0.1331 ± 0.0012            & \multicolumn{1}{l|}{0.1703 ± 0.0018} & 0.7170 ± 0.0011           & 0.7169 ± 0.0013           & 0.5226 ± 0.0054          & 0.7082 ± 0.001          & 0.9996 ± 0.0001         & 0.7847 ± 0.0148          & 0.9083 ± 0.0013            \\
                                    & uci                  & 0.8397 ± 0.0006           & 0.9165 ± 0.0016            & 0.8383 ± 0.0001           & 0.7245 ± 0.0034            & \multicolumn{1}{l|}{0.9293 ± 0.0006} & 0.4771 ± 0.0100           & 0.6393 ± 0.0158           & 0.7680 ± 0.0041          & 0.8051 ± 0.021          & 0.9472 ± 0.0262         & 0.9245 ± 0.0027          & 0.9716 ± 0.0016            \\
                                    & untrade              & 0.7036 ± 0.0059           & 0.5541 ± 0.0028            & 0.7028 ± 0.0095           & 0.2621 ± 0.0144            & \multicolumn{1}{l|}{}                & 0.5362 ± 0.0147           & 0.5922 ± 0.0085           &                          & 0.5068 ± 0.0061         & 0.6876 ± 0.0177         & 0.7458 ± 0.0081          & 0.5938 ± 0.0600            \\
                                    & unvote               & 0.6345 ± 0.0022           & 0.5162 ± 0.0008            & 0.6149 ± 0.0026           & 0.1448 ± 0.0041            & \multicolumn{1}{l|}{}                & 0.4728 ± 0.0033           & 0.4913 ± 0.0203           & 0.5000 ± 0.006           & 0.5663 ± 0.0093         & 0.7198 ± 0.0748         & 0.5775 ± 0.0022          & 0.5669 ± 0.0               \\
                                    & uslegis              & 0.5379 ± 0.0041           & 0.4901 ± 0.0032            & 0.5376 ± 0.0041           & 0.1748 ± 0.003             & \multicolumn{1}{l|}{}                & 0.5640 ± 0.0192           & 0.5390 ± 0.0075           & 0.5324 ± 0.0294          & 0.5626 ± 0.0195         & 0.8897 ± 0.0225         & 0.9738 ± 0.0058          & 0.9787 ± 0.0004            \\
                                    & wikipedia            & 0.9403 ± 0.0003           & 0.9286 ± 0.0011            & 0.9403 ± 0.0002           & 0.352 ± 0.0018             & \multicolumn{1}{l|}{0.9764 ± 0.0005} & 0.9261 ± 0.0030           & 0.9349 ± 0.0051           & 0.9580 ± 0.0039          & 0.9858 ± 0.0007         & 0.9984 ± 0.0008         & 0.9934 ± 0.0005          & 0.9960 ± 0.0001            \\
\multirow{15}{*}{inductive new old} & canparl              & 0.6587 ± 0.0008           & 0.6414 ± 0.0017            & 0.6556 ± 0.0011           & 0.6447 ± 0.0036            & \multicolumn{1}{l|}{0.6475 ± 0.0023} & 0.5393 ± 0.0204           & 0.5078 ± 0.0005           & 0.5724 ± 0.0063          & 0.5691 ± 0.0223         & 0.6277 ± 0.0811         & 0.7231 ± 0.085           & 0.8847 ± 0.0102            \\
                                    & collegemsg           & 0.8353 ± 0.0005           & 0.9214 ± 0.0026            & 0.8324 ± 0.0006           & 0.8074 ± 0.003             & \multicolumn{1}{l|}{0.9329 ± 0.0002} & 0.4808 ± 0.0279           & 0.5168 ± 0.0360           & 0.7012 ± 0.005           & 0.7725 ± 0.0365         & 0.9725 ± 0.0189         & 0.9166 ± 0.0032          & 0.968 ± 0.0018             \\
                                    & contact              & 0.9656 ± 0.0003           & 0.8756 ± 0.0004            & 0.9377 ± 0.0004           & 0.6317 ± 0.0011            & \multicolumn{1}{l|}{0.9776 ± 0.0002} & 0.8574 ± 0.0454           & 0.9345 ± 0.0027           & 0.556 ± 0.0039           & 0.9527 ± 0.0052         & 0.9351 ± 0.0202         & 0.9691 ± 0.0028          & 0.9841 ± 0.0               \\
                                    & enron                & 0.9126 ± 0.001            & 0.8171 ± 0.0023            & 0.9041 ± 0.0031           & 0.5593 ± 0.0052            & \multicolumn{1}{l|}{0.9366 ± 0.0013} & 0.6915 ± 0.0650           & 0.7859 ± 0.0134           & 0.5589 ± 0.0235          & 0.8100 ± 0.0204         & 0.9491 ± 0.0079         & 0.9185 ± 0.003           & 0.9007 ± 0.0039            \\
                                    & flights              & 0.8486 ± 0.0002           & 0.7858 ± 0.0011            & 0.8474 ± 0.0001           & 0.8386 ± 0.0004            & \multicolumn{1}{l|}{0.9276 ± 0.0002} & 0.8650 ± 0.0126           & 0.9172 ± 0.0114           & 0.8285 ± 0.0038          & 0.9503 ± 0.0043         & 0.986 ± 0.0034          & 0.9828 ± 0.0002          & 0.9127 ± 0.0               \\
                                    & lastfm               & 0.8676 ± 0.0006           & 0.6764 ± 0.0007            & 0.8463 ± 0.0002           & 0.4862 ± 0.0008            & \multicolumn{1}{l|}{0.8766 ± 0.0003} & 0.6980 ± 0.0364           & 0.7305 ± 0.0051           & 0.5189 ± 0.003           & 0.7630 ± 0.0231         & 0.9144 ± 0.0013         & 0.8678 ± 0.0030          & 0.8311 ± 0.0               \\
                                    & mooc                 & 0.6666 ± 0.0003           & 0.6972 ± 0.0007            & 0.6165 ± 0.0002           & 0.5626 ± 0.0016            & \multicolumn{1}{l|}{0.7091 ± 0.0005} & 0.8274 ± 0.0132           & 0.7910 ± 0.0475           & 0.7438 ± 0.0063          & 0.8808 ± 0.0326         & 0.7487 ± 0.0459         & 0.9490 ± 0.0016          & 0.8052 ± 0.0244            \\
                                    & reddit               & 0.9545 ± 0.0              & 0.8926 ± 0.0487            & 0.9545 ± 0.0              & 0.741 ± 0.0666             & \multicolumn{1}{l|}{0.9945 ± 0.0078} & 0.9549 ± 0.0029           & 0.9488 ± 0.0043           & 0.9639 ± 0.0004          & 0.9742 ± 0.0004         & 0.9949 ± 0.0017         & 0.9848 ± 0.0002          & 0.9789 ± 0.0017            \\
                                    & socialevo            & 0.9519 ± 0.0002           & 0.7857 ± 0.0003            & 0.8583 ± 0.0005           & 0.4987 ± 0.0013            & \multicolumn{1}{l|}{0.952 ± 0.001}   & 0.9182 ± 0.0050           & 0.8953 ± 0.0303           & 0.6840 ± 0.0034          & 0.9257 ± 0.0086         & 0.8793 ± 0.0318         & 0.9155 ± 0.0002          &                            \\
                                    & taobao               & 0.521 ± 0.0               & 0.2699 ± 0.002             & 0.5209 ± 0.0001           & 0.2797 ± 0.0015            & \multicolumn{1}{l|}{0.2759 ± 0.0008} & 0.6992 ± 0.0001           & 0.6988 ± 0.0024           & 0.5266 ± 0.0239          & 0.7025 ± 0.0038         & 0.9997 ± 0.0001         & 0.7574 ± 0.0032          & 0.8617 ± 0.0032            \\
                                    & uci                  & 0.8329 ± 0.0003           & 0.9209 ± 0.0014            & 0.8305 ± 0.0004           & 0.8034 ± 0.0044            & \multicolumn{1}{l|}{0.9333 ± 0.0005} & 0.4259 ± 0.0397           & 0.7139 ± 0.0112           & 0.6842 ± 0.0078          & 0.8015 ± 0.0269         & 0.9748 ± 0.0163         & 0.9176 ± 0.0028          & 0.9696 ± 0.0039            \\
                                    & untrade              & 0.6892 ± 0.0009           & 0.552 ± 0.0009             & 0.5841 ± 0.0018           & 0.4881 ± 0.0031            & \multicolumn{1}{l|}{}                & 0.6306 ± 0.0139           & 0.6650 ± 0.0106           &                          & 0.5959 ± 0.0171         & 0.5812 ± 0.0957         & 0.7413 ± 0.001           & 0.5965 ± 0.0371            \\
                                    & unvote               & 0.6385 ± 0.0015           & 0.5169 ± 0.0001            & 0.4893 ± 0.0007           & 0.3886 ± 0.0003            & \multicolumn{1}{l|}{}                & 0.5023 ± 0.0204           & 0.5208 ± 0.0075           & 0.4787 ± 0.0033          & 0.5889 ± 0.0106         & 0.7789 ± 0.0192         & 0.5933 ± 0.0007          & 0.5878 ± 0.0               \\
                                    & uslegis              & 0.5901 ± 0.004            & 0.641 ± 0.0017             & 0.54 ± 0.004              & 0.4432 ± 0.0038            & \multicolumn{1}{l|}{}                & 0.5673 ± 0.0098           & 0.5801 ± 0.0213           & 0.5596 ± 0.0092          & 0.5741 ± 0.0148         & 0.5310 ± 0.1            & 0.9672 ± 0.0029          & 0.9682 ± 0.0018            \\
                                    & wikipedia            & 0.9072 ± 0.0001           & 0.9104 ± 0.0008            & 0.9064 ± 0.0001           & 0.4656 ± 0.0018            & \multicolumn{1}{l|}{0.957 ± 0.0006}  & 0.8821 ± 0.0031           & 0.9084 ± 0.0043           & 0.9178 ± 0.0023          & 0.9703 ± 0.0008         & 0.9963 ± 0.0021         & 0.9886 ± 0.0002          & 0.9878 ± 0.0002            \\
\multirow{15}{*}{transductive}      & canparl              & 0.7237 ± 0.0003           & 0.7221 ± 0.0012            & 0.7227 ± 0.0007           & 0.7172 ± 0.0028            & \multicolumn{1}{l|}{0.7313 ± 0.0003} & 0.7737 ± 0.0255           & 0.7939 ± 0.0063           & 0.7077 ± 0.0218          & 0.7575 ± 0.0694         & 0.6917 ± 0.0722         & 0.7197 ± 0.0905          & 0.8920 ± 0.0173            \\
                                    & collegemsg           & 0.8722 ± 0.0003           & 0.9233 ± 0.0013            & 0.8697 ± 0.0004           & 0.8747 ± 0.001             & \multicolumn{1}{l|}{0.9512 ± 0.0019} & 0.5382 ± 0.0058           & 0.5730 ± 0.0690           & 0.8084 ± 0.0032          & 0.8419 ± 0.084          & 0.9059 ± 0.0122         & 0.9156 ± 0.004           & 0.9698 ± 0.0               \\
                                    & contact              & 0.9764 ± 0.0001           & 0.8776 ± 0.0001            & 0.9557 ± 0.0              & 0.7941 ± 0.0001            & \multicolumn{1}{l|}{0.9821 ± 0.0001} & 0.9276 ± 0.0206           & 0.9379 ± 0.0073           & 0.5582 ± 0.009           & 0.9769 ± 0.0032         & 0.9463 ± 0.021          & 0.9685 ± 0.0028          & 0.9840 ± 0.0               \\
                                    & enron                & 0.9036 ± 0.0005           & 0.8183 ± 0.0016            & 0.896 ± 0.0005            & 0.6898 ± 0.0029            & \multicolumn{1}{l|}{0.9286 ± 0.0006} & 0.7986 ± 0.0358           & 0.8293 ± 0.0148           & 0.6161 ± 0.0214          & 0.8621 ± 0.0173         & 0.9212 ± 0.0029         & 0.9159 ± 0.0032          & 0.8956 ± 0.0045            \\
                                    & flights              & 0.9213 ± 0.0001           & 0.7938 ± 0.0003            & 0.9217 ± 0.0001           & 0.9072 ± 0.0001            & \multicolumn{1}{l|}{0.965 ± 0.0}     & 0.8981 ± 0.0056           & 0.9449 ± 0.0073           & 0.9016 ± 0.0027          & 0.9787 ± 0.0025         & 0.9747 ± 0.0061         & 0.9861 ± 0.0002          & 0.9302 ± 0.0               \\
                                    & lastfm               & 0.8946 ± 0.0004           & 0.62 ± 0.0009              & 0.8719 ± 0.0004           & 0.6152 ± 0.0004            & \multicolumn{1}{l|}{0.8987 ± 0.0001} & 0.6793 ± 0.0553           & 0.6766 ± 0.0590           & 0.5094 ± 0.0071          & 0.7743 ± 0.0256         & 0.8536 ± 0.0027         & 0.8746 ± 0.0013          & 0.8390 ± 0.0               \\
                                    & mooc                 & 0.7279 ± 0.0011           & 0.7414 ± 0.001             & 0.6501 ± 0.0014           & 0.6741 ± 0.0014            & \multicolumn{1}{l|}{0.7682 ± 0.0009} & 0.8243 ± 0.0323           & 0.7899 ± 0.0208           & 0.7391 ± 0.0056          & 0.8999 ± 0.0213         & 0.7568 ± 0.0305         & 0.9459 ± 0.0008          & 0.8071 ± 0.0193            \\
                                    & reddit               & 0.9584 ± 0.0001           & 0.8814 ± 0.0001            & 0.9584 ± 0.0001           & 0.8978 ± 0.0005            & \multicolumn{1}{l|}{0.9758 ± 0.0}    & 0.9803 ± 0.0005           & 0.9760 ± 0.0006           & 0.9810 ± 0.0002          & 0.9871 ± 0.0001         & 0.9854 ± 0.002          & 0.9891 ± 0.0000          & 0.9841 ± 0.0016            \\
                                    & socialevo            & 0.9574 ± 0.0001           & 0.7829 ± 0.0005            & 0.9075 ± 0.0              & 0.7238 ± 0.0005            & \multicolumn{1}{l|}{0.9574 ± 0.0003} & 0.9020 ± 0.0026           & 0.8666 ± 0.0233           & 0.7851 ± 0.0047          & 0.9520 ± 0.0003         & 0.9202 ± 0.0065         & 0.9337 ± 0.0003          &                            \\
                                    & taobao               & 0.6635 ± 0.0              & 0.6169 ± 0.0084            & 0.6635 ± 0.0              & 0.752 ± 0.006              & \multicolumn{1}{l|}{0.7438 ± 0.004}  & 0.8409 ± 0.0012           & 0.8405 ± 0.0006           & 0.5396 ± 0.009           & 0.8654 ± 0.0005         & 0.8937 ± 0.0015         & 0.7708 ± 0.0026          & 0.8759 ± 0.0009            \\
                                    & uci                  & 0.8752 ± 0.0002           & 0.9258 ± 0.0013            & 0.8722 ± 0.0003           & 0.8774 ± 0.0029            & \multicolumn{1}{l|}{0.9541 ± 0.0013} & 0.5086 ± 0.0651           & 0.8786 ± 0.0017           & 0.7998 ± 0.0052          & 0.8875 ± 0.0161         & 0.9076 ± 0.0116         & 0.9189 ± 0.0017          & 0.9670 ± 0.0031            \\
                                    & untrade              & 0.6936 ± 0.0008           & 0.554 ± 0.0006             & 0.7194 ± 0.0008           & 0.7196 ± 0.0013            & \multicolumn{1}{l|}{}                & 0.6377 ± 0.0032           & 0.6786 ± 0.0103           &                          & 0.6543 ± 0.01           & 0.783 ± 0.0472          & 0.7511 ± 0.0012          & 0.5924 ± 0.0368            \\
                                    & unvote               & 0.6468 ± 0.0006           & 0.5194 ± 0.0001            & 0.6763 ± 0.0006           & 0.643 ± 0.0007             & \multicolumn{1}{l|}{}                & 0.6236 ± 0.0305           & 0.6523 ± 0.0082           & 0.5134 ± 0.0026          & 0.7176 ± 0.0109         & 0.6776 ± 0.0411         & 0.6037 ± 0.0019          & 0.5871 ± 0.0               \\
                                    & uslegis              & 0.7711 ± 0.0072           & 0.7751 ± 0.0043            & 0.746 ± 0.0064            & 0.6946 ± 0.0093            & \multicolumn{1}{l|}{}                & 0.7425 ± 0.0374           & 0.8278 ± 0.0024           & 0.7738 ± 0.0062          & 0.8137 ± 0.002          & 0.7820 ± 0.0261         & 0.9643 ± 0.0043          & 0.9715 ± 0.0009            \\
                                    & wikipedia            & 0.9634 ± 0.0003           & 0.9055 ± 0.0003            & 0.9631 ± 0.0002           & 0.6724 ± 0.0021            & \multicolumn{1}{l|}{0.9825 ± 0.0001} & 0.9426 ± 0.0007           & 0.9505 ± 0.0032           & 0.9509 ± 0.0017          & 0.9846 ± 0.0003         & 0.9786 ± 0.0035         & 0.9889 ± 0.0             & 0.9912 ± 0.0001            \\ \bottomrule
\end{tabular}%
}

==> full_mrr.tex <==
\begin{tabular}{lllll}
\toprule
Split &          Valid &           Test &         Valid &          Test \\
Tracker & Global Recency & Global Recency & Local Recency & Local Recency \\
Dataset            &                &                &               &               \\
\midrule
CanParl            &          0.025 &          0.034 &         0.056 &         0.054 \\
CollegeMsg         &          0.134 &          0.154 &         0.417 &         0.468 \\
Contacts           &          0.016 &          0.016 &         0.718 &         0.684 \\
DGraphFin          &          0.000 &          0.000 &         0.000 &         0.000 \\
Flights            &          0.000 &          0.000 &         0.133 &         0.130 \\
SocialEvo          &          0.132 &          0.138 &         0.747 &         0.786 \\
TaobaoLarge        &          0.000 &          0.000 &         0.055 &         0.055 \\
UNtrade            &          0.044 &          0.031 &         0.205 &         0.202 \\
UNvote             &          0.076 &          0.073 &         0.539 &         0.570 \\
USLegis            &          0.055 &          0.046 &         0.062 &         0.058 \\
YoutubeRedditLarge &          0.017 &          0.044 &         0.103 &         0.298 \\
enron              &          0.143 &          0.161 &         0.551 &         0.537 \\
lastfm             &          0.036 &          0.040 &         0.174 &         0.166 \\
mooc               &          0.135 &          0.142 &         0.305 &         0.318 \\
reddit             &          0.096 &          0.097 &         0.715 &         0.716 \\
taobao             &          0.000 &          0.000 &         0.034 &         0.036 \\
tgbl-coin          &          0.022 &          0.023 &         0.397 &         0.411 \\
tgbl-comment       &          0.005 &          0.004 &         0.086 &         0.085 \\
tgbl-flight        &          0.000 &          0.000 &         0.131 &         0.130 \\
tgbl-lastfm        &          0.036 &          0.040 &         0.174 &         0.166 \\
tgbl-review        &          0.000 &          0.000 &         0.001 &         0.001 \\
tgbl-subreddit     &          0.096 &          0.097 &         0.715 &         0.716 \\
tgbl-wiki          &          0.140 &          0.157 &         0.839 &         0.817 \\
uci                &          0.134 &          0.154 &         0.417 &         0.468 \\
wikipedia          &          0.140 &          0.157 &         0.839 &         0.817 \\
\bottomrule
\end{tabular}

==> results_table_old.tex <==
\begin{tabular}{lllllllll}
\toprule
% Heuristic & LR-GR-LP-GP &         LR-GR & LR-GP &        LR-LP-GR & \multicolumn{2}{l}{Popularity} & \multicolumn{2}{l}{Recency} \\
{Dataset~/~Heuristic} & LR-GR-LP-GP & LR-GR & LR-LP-GR &     GP & LP & GP & LP \\
\midrule
\textbf{tgbl-coin}      &                 0.809 (1)&                              0.808 (1) &                                               0.809  (1) &      0.613 (3) &  0.692 (3) &   0.726 (3) &  0.773 (1) \\
\textbf{tgbl-comment}   &          0.455 (3)            &                              0.455 (3) &    0.455 (3)                                                 &      0.354 (4) &  0.106 (7) &   0.723 (1) &  0.164 (5) \\
\textbf{tgbl-flight}    &                  0.88 (1) &                              0.833 (1) &                                                  0.88 (1) &      0.603 (3) &  0.871 (1) &   0.183 &  0.831 (1) \\
% tgbl-lastfm    &                 0.166 &                              0.166 &                0.166 &                                              0.166 &      0.013 &  0.107 &    0.04 &  0.166 \\
\textbf{tgbl-review}    &                 0.199 &                              0.196 &                                                          0.196 &      0.321 &  0.001 &   0.394 &  0.001 \\
% tgbl-subreddit &                 0.717 &                              0.717 &                0.718 &                                              0.717 &      0.193 &  0.738 &   0.097 &  0.716 \\
\textbf{tgbl-wiki}      &                 0.821 (1) &                              0.821 (1) &                                                           0.821 (1) &       0.04 (12) &  0.693 (5) &   0.157 (9) &  {0.817} (1) \\
\bottomrule
\end{tabular}

==> temporal_incoherence.tex <==
When recency serves as the sole predictor, it provides a straightforward means to quantify its importance. Since the heuristics rely exclusively on recency, batching inherently leads to a measurable loss of information, as temporally dependent edges are grouped together. This effect is especially significant in the context of local recency. We provide a theoretical proof of this statement in Appendix~\ref{sec:batching_incoherency}.

\section{Fixed Batch Size and Temporal Incoherence}
\label{sec:batching_incoherency}

\noindent
\textbf{Theorem.} A model that processes edges in fixed-size batches is inherently temporally incoherent unless each batch exactly aligns with a unique, consecutive set of timestamps and all but the final batch contain exactly $B$ edges. Formally, let $E = \{(u,v,t)\mid u,v \in V,\, t\in T\subseteq \mathbb{N}\}$, and let $E_t$ be the set of edges occurring at time $t$. Then any batching scheme that groups edges into subsets $b_i \subset E$ of fixed size $B$ is temporally incoherent unless all timestamps in each subset are strictly greater than all timestamps in any previous subset.

\medskip

\noindent
\textbf{Definition (Temporal Incoherence).} A batching scheme is called \emph{temporally incoherent} if there exist batches $b_i$ and $b_{i+j}$ such that
$$
\max_{(u,v,t)\in b_i} t \;\;\ge\;\; \min_{(u,v,t)\in b_{i+j}} t,
$$
meaning edges in a later batch include timestamps not strictly greater than those in the earlier batch.

\medskip

\noindent
\textbf{Proof.}
We first note that edges may be grouped by their timestamps: $E = \bigcup_{t \in T} E_t,$ where $E_t = \{(u,v,t) \mid u,v \in V\}$. We sort these sets in ascending order of $t$. Suppose a scheme attempts to form batches of size $B$.

\paragraph{Case 1: $\max_t |E_t| > B$.}
If there exists a timestamp $t$ such that $|E_t|>B$, then any single batch cannot contain all edges from time $t$. This forces us to split $E_t$ into at least two batches, both of which include edges with the same timestamp. Hence,
$$
\max_{b_i} t \;=\; t \quad\text{and}\quad \min_{b_{i+1}} t \;\le\; t,
$$
causing temporal incoherence.

\paragraph{Case 2: $\max_t |E_t|\le B$.}
When each $E_t$ can fit into a batch of size $B$, the batching scheme typically groups consecutive timestamps together until the batch reaches size $B$. Formally, we can write
$$
b_i \;=\; \bigcup_{t = t_{s_i}}^{t_{e_i}} E_t,
$$
where $|b_i| = B$ (except possibly the last batch). If the end time $t_{e_i}$ of one batch is greater than or equal to the start time $t_{s_{i+1}} \ge t_{e_i}$ of the next batch, we again have
$$
\max_{(u,v,t)\in b_i} t \;\;\ge\;\; \min_{(u,v,t)\in b_{i+1}} t,
$$
leading to temporal incoherence unless the boundaries align perfectly so that each timestamp lies entirely within a single batch. This perfect alignment can only happen if the counts of edges at consecutive timestamps sum exactly to \(B\) (for all batches except possibly the last) and no timestamp is split across batches.

In either scenario, the only way to preserve strict temporal ordering with a fixed batch size $B$ is to have each timestamp $t$ fully contained in exactly one batch, and for the number of edges at consecutive timestamps to sum up to $B$ precisely until the final subset of edges is reached. This special case requires a strict partition of $E$ by timestamps without overlap, which is generally infeasible unless the dataset is constructed to fit these constraints exactly.$~\square$

